Irrelevance of personalized pricing under strategic market segmentation

A multiproduct seller is more informed than consumers about the value of her products to consumers. The seller posts a price list and segments the market through cheap-talk communication. We find that when both seller's and consumers' incentive-compatibility constraints are satisfied, the seller cannot benefit from personalized pricing (i.e., third-degree price discrimination). Based on that observation, we provide a tractable characterization of seller's maximum equilibrium profits. We apply our analysis to a credence-good setup and discuss when the credence goods seller benefits from communication. The irrelevance result breaks down when we relax seller's incentive-compatibility constraints.

==> preamble.tex <==
% fig env
\usepackage{changepage}
% \usepackage[margin=2cm]{caption}
\newenvironment{fig}%
  {\begin{figure}%
    \begin{adjustwidth}{-2cm}{-2cm}%
    \begin{center}%
    \captionsetup{margin=3cm}}%
  {\end{center}%
    \end{adjustwidth}%
    \end{figure}}

% PDF string definitions for hyperref
\pdfstringdefDisableCommands{%
  \def\\{}%
  \def\texttt#1{<#1>}%
  \def\Cref#1{<#1>}%
}



% Define the command and variable
\newcommand\thx[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{ #1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

% AMS theorem environments
\newtheorem{lmm}{Lemma}
\newtheorem{thm}{Theorem}
\newtheorem{prp}{Proposition}

\theoremstyle{definition}
\newtheorem{dfn}{Definition}
\newtheorem{eg}{Example}
\newtheorem{clm}{Claim}

\theoremstyle{remark}
\newtheorem*{rmk}{rmk}
\newtheorem{crl}{Corollary}






% put unicodes here
\RequirePackage{newunicodechar}
\newunicodechar{ℂ}{\ensuremath{\mathbb{C}}}
% A collection of `\newunicodechar` declarations.
% Adapted from https://github.com/armkeh/unicode-sty/tree/master

\newunicodechar{ℍ}{\ensuremath{\mathbb{H}}}

\newunicodechar{ℕ}{\ensuremath{\mathbb{N}}}

\newunicodechar{ℙ}{\ensuremath{\mathbb{P}}}
\newunicodechar{ℚ}{\ensuremath{\mathbb{Q}}}
\newunicodechar{ℝ}{\ensuremath{\mathbb{R}}}

\newunicodechar{ℤ}{\ensuremath{\mathbb{Z}}}

% For double stroke digits with pdflatex
% \RequirePackage[bbgreekl]{mathbbol}
% \DeclareSymbolFontAlphabet{\mathbbl}{bbold}







\newunicodechar{ℓ}{\ensuremath{\ell}}
\newunicodechar{α}{\ensuremath{\alpha}}
\newunicodechar{β}{\ensuremath{\beta}}
\newunicodechar{γ}{\ensuremath{\gamma}}
\newunicodechar{Γ}{\ensuremath{\Gamma}}
\newunicodechar{δ}{\ensuremath{\delta}}
\newunicodechar{Δ}{\ensuremath{\Delta}}
\newunicodechar{ϵ}{\ensuremath{\epsilon}}
\newunicodechar{ζ}{\ensuremath{\zeta}}
\newunicodechar{η}{\ensuremath{\eta}}
\newunicodechar{∑}{\ensuremath{\sum}}
\newunicodechar{θ}{\ensuremath{\theta}}
\newunicodechar{Θ}{\ensuremath{\Theta}}
\newunicodechar{ι}{\ensuremath{\iota}}
\newunicodechar{κ}{\ensuremath{\kappa}}
\newunicodechar{λ}{\ensuremath{\lambda}}
\newunicodechar{Λ}{\ensuremath{\Lambda}}
\newunicodechar{μ}{\ensuremath{\mu}}
\newunicodechar{ν}{\ensuremath{\nu}}
\newunicodechar{ξ}{\ensuremath{\xi}}
\newunicodechar{Ξ}{\ensuremath{\Xi}}

\newunicodechar{π}{\ensuremath{\pi}}
\newunicodechar{Π}{\ensuremath{\Pi}}
\newunicodechar{ρ}{\ensuremath{\rho}}
\newunicodechar{𝔼}{\ensuremath{\mathbb{E}}}



\newunicodechar{σ}{\ensuremath{\sigma}}
\newunicodechar{Σ}{\ensuremath{\Sigma}}
\newunicodechar{τ}{\ensuremath{\tau}}

\newunicodechar{υ}{\ensuremath{\upsilon}}
\newunicodechar{Υ}{\ensuremath{\Upsilon}}
\newunicodechar{ϕ}{\ensuremath{\phi}}
\newunicodechar{Φ}{\ensuremath{\Phi}}
\newunicodechar{χ}{\ensuremath{\chi}}

\newunicodechar{ψ}{\ensuremath{\psi}}
\newunicodechar{Ψ}{\ensuremath{\Psi}}
\newunicodechar{ω}{\ensuremath{\omega}}
\newunicodechar{Ω}{\ensuremath{\Omega}}

\newunicodechar{ε}{\ensuremath{\varepsilon}}
\newunicodechar{ϑ}{\ensuremath{\vartheta}}
\newunicodechar{ϰ}{\ensuremath{\varkappa}}
\newunicodechar{ϖ}{\ensuremath{\varpi}}
\newunicodechar{ς}{\ensuremath{\varsigma}}
\newunicodechar{φ}{\ensuremath{\varphi}}

\newunicodechar{ₐ}{\ensuremath{{}_{a}}}
\newunicodechar{ₑ}{\ensuremath{{}_{e}}}
\newunicodechar{ₕ}{\ensuremath{{}_{h}}}
\newunicodechar{ᵢ}{\ensuremath{{}_{i}}}
\newunicodechar{ⱼ}{\ensuremath{{}_{j}}}
\newunicodechar{ₖ}{\ensuremath{{}_{k}}}
\newunicodechar{ₗ}{\ensuremath{{}_{l}}}
\newunicodechar{ₘ}{\ensuremath{{}_{m}}}
\newunicodechar{ₙ}{\ensuremath{{}_{n}}}
\newunicodechar{ₒ}{\ensuremath{{}_{o}}}
\newunicodechar{ₚ}{\ensuremath{{}_{p}}}
\newunicodechar{ᵣ}{\ensuremath{{}_{r}}}
\newunicodechar{ₛ}{\ensuremath{{}_{s}}}
\newunicodechar{ₜ}{\ensuremath{{}_{t}}}
\newunicodechar{ᵤ}{\ensuremath{{}_{u}}}
\newunicodechar{ᵥ}{\ensuremath{{}_{v}}}
\newunicodechar{ₓ}{\ensuremath{{}_{x}}}

\newunicodechar{₀}{\ensuremath{{}_{0}}}
\newunicodechar{₁}{\ensuremath{{}_{1}}}
\newunicodechar{₂}{\ensuremath{{}_{2}}}
\newunicodechar{₃}{\ensuremath{{}_{3}}}
\newunicodechar{₄}{\ensuremath{{}_{4}}}
\newunicodechar{₅}{\ensuremath{{}_{5}}}
\newunicodechar{₆}{\ensuremath{{}_{6}}}
\newunicodechar{₇}{\ensuremath{{}_{7}}}
\newunicodechar{₈}{\ensuremath{{}_{8}}}
\newunicodechar{₉}{\ensuremath{{}_{9}}}

\newunicodechar{₊}{\ensuremath{{}_{+}}}
\newunicodechar{₋}{\ensuremath{{}_{-}}}
\newunicodechar{₌}{\ensuremath{{}_{=}}}

\newunicodechar{ᴬ}{\ensuremath{{}^{A}}}
\newunicodechar{ᴮ}{\ensuremath{{}^{B}}}
\newunicodechar{ᴰ}{\ensuremath{{}^{D}}}
\newunicodechar{ᴱ}{\ensuremath{{}^{E}}}
\newunicodechar{ᴳ}{\ensuremath{{}^{G}}}
\newunicodechar{ᴴ}{\ensuremath{{}^{H}}}
\newunicodechar{ᴵ}{\ensuremath{{}^{I}}}
\newunicodechar{ᴶ}{\ensuremath{{}^{J}}}
\newunicodechar{ᴷ}{\ensuremath{{}^{K}}}
\newunicodechar{ᴸ}{\ensuremath{{}^{L}}}
\newunicodechar{ᴹ}{\ensuremath{{}^{M}}}
\newunicodechar{ᴺ}{\ensuremath{{}^{N}}}
\newunicodechar{ᴼ}{\ensuremath{{}^{O}}}
\newunicodechar{ᴾ}{\ensuremath{{}^{P}}}
\newunicodechar{ᴿ}{\ensuremath{{}^{R}}}
\newunicodechar{ᵀ}{\ensuremath{{}^{T}}}
\newunicodechar{ᵁ}{\ensuremath{{}^{U}}}
\newunicodechar{ⱽ}{\ensuremath{{}^{V}}}
\newunicodechar{ᵂ}{\ensuremath{{}^{W}}}

\newunicodechar{ᵃ}{\ensuremath{{}^{a}}}
\newunicodechar{ᵇ}{\ensuremath{{}^{b}}}
\newunicodechar{ᶜ}{\ensuremath{{}^{c}}}
\newunicodechar{ᵈ}{\ensuremath{{}^{d}}}
\newunicodechar{ᵉ}{\ensuremath{{}^{e}}}
\newunicodechar{ᶠ}{\ensuremath{{}^{f}}}
\newunicodechar{ᵍ}{\ensuremath{{}^{g}}}
\newunicodechar{ʰ}{\ensuremath{{}^{h}}}
\newunicodechar{ⁱ}{\ensuremath{{}^{i}}}
\newunicodechar{ʲ}{\ensuremath{{}^{j}}}
\newunicodechar{ᵏ}{\ensuremath{{}^{k}}}
\newunicodechar{ˡ}{\ensuremath{{}^{l}}}
\newunicodechar{ᵐ}{\ensuremath{{}^{m}}}
\newunicodechar{ⁿ}{\ensuremath{{}^{n}}}
\newunicodechar{ᵒ}{\ensuremath{{}^{o}}}
\newunicodechar{ᵖ}{\ensuremath{{}^{p}}}
\newunicodechar{ʳ}{\ensuremath{{}^{r}}}
\newunicodechar{ˢ}{\ensuremath{{}^{s}}}
\newunicodechar{ᵗ}{\ensuremath{{}^{t}}}
\newunicodechar{ᵘ}{\ensuremath{{}^{u}}}
\newunicodechar{ᵛ}{\ensuremath{{}^{v}}}
\newunicodechar{ʷ}{\ensuremath{{}^{w}}}
\newunicodechar{ˣ}{\ensuremath{{}^{x}}}
\newunicodechar{ʸ}{\ensuremath{{}^{y}}}
\newunicodechar{ᶻ}{\ensuremath{{}^{z}}}

\newunicodechar{⁰}{\ensuremath{{}^{0}}}
% \newunicodechar{¹}{\ensuremath{{}^{1}}}
% \newunicodechar{²}{\ensuremath{{}^{2}}}
% \newunicodechar{³}{\ensuremath{{}^{3}}}
\newunicodechar{⁴}{\ensuremath{{}^{4}}}
\newunicodechar{⁵}{\ensuremath{{}^{5}}}
\newunicodechar{⁶}{\ensuremath{{}^{6}}}
\newunicodechar{⁷}{\ensuremath{{}^{7}}}
\newunicodechar{⁸}{\ensuremath{{}^{8}}}
\newunicodechar{⁹}{\ensuremath{{}^{9}}}

\newunicodechar{⁺}{\ensuremath{{}^{+}}}
\newunicodechar{⁻}{\ensuremath{{}^{-}}}
\newunicodechar{⁼}{\ensuremath{{}^{=}}}

\newunicodechar{…}{\ensuremath{\ldots}}
\newunicodechar{⋯}{\ensuremath{\cdots}}
\newunicodechar{⋮}{\ensuremath{\vdots}}

\newunicodechar{–}{\ensuremath{\text{--}}}
\newunicodechar{—}{\ensuremath{\text{---}}}

\newunicodechar{◻}{\ensuremath{\square}}



\newunicodechar{⦅}{\ensuremath{(\!|}}
\newunicodechar{⦆}{\ensuremath{|\!)}}
\newunicodechar{⟨}{\ensuremath{\langle}}
\newunicodechar{⟩}{\ensuremath{\rangle}}
\newunicodechar{⦃}{\ensuremath{\{\!\mid}}
\newunicodechar{⦄}{\ensuremath{\mid\!\}}}
\newunicodechar{⟪}{\ensuremath{\langle\!\langle}}
\newunicodechar{⟫}{\ensuremath{\rangle\!\rangle}}
\newunicodechar{⁅}{\ensuremath{\{}}
\newunicodechar{⁆}{\ensuremath{\}}}
\newunicodechar{｛}{\ensuremath{\{}}
\newunicodechar{｝}{\ensuremath{\}}}

\newunicodechar{⟦}{\ensuremath{[\![}}
\newunicodechar{⟧}{\ensuremath{]\!]}}

\newunicodechar{⌜}{\ensuremath{\ulcorner}}
\newunicodechar{⌝}{\ensuremath{\urcorner}}
\newunicodechar{⌞}{\ensuremath{\llcorner}}
\newunicodechar{⌟}{\ensuremath{\lrcorner}}
\newunicodechar{⌈}{\ensuremath{\lceil}}
\newunicodechar{⌉}{\ensuremath{\rceil}}
\newunicodechar{⌊}{\ensuremath{\lfloor}}
\newunicodechar{⌋}{\ensuremath{\rfloor}}

% \newunicodechar{∼}{\ensuremath{~}} 

\newunicodechar{≡}{\ensuremath{\equiv}}
\newunicodechar{¬}{\ensuremath{\lnot}}
\newunicodechar{≢}{\ensuremath{\not\equiv}}
\newunicodechar{∨}{\ensuremath{\lor}}
\newunicodechar{∧}{\ensuremath{\land}}
\newunicodechar{⇒}{\ensuremath{\;\Rightarrow\;}}
\newunicodechar{⇐}{\ensuremath{\;\Leftarrow\;}}
\newunicodechar{⟺}{\ensuremath{\iff}}
\newunicodechar{⇔}{\ensuremath{\iff}}

\newunicodechar{∀}{\ensuremath{\forall}}
\newunicodechar{∃}{\ensuremath{\exists}}

\newunicodechar{❙}{\ensuremath{\,\mid\,}}
\newunicodechar{•}{\ensuremath{\,\bullet\,}}

\newunicodechar{⊢}{\ensuremath{\vdash}}
\newunicodechar{⊣}{\ensuremath{\dashv}}
\newunicodechar{⊨}{\ensuremath{\vDash}}

\newunicodechar{ø}{\ensuremath{\emptyset}}
\newunicodechar{∅}{\ensuremath{\emptyset}}
\newunicodechar{∈}{\ensuremath{\in}}
\newunicodechar{∉}{\ensuremath{\not\in}}
\newunicodechar{∋}{\ensuremath{\ni}}
\newunicodechar{⊆}{\ensuremath{\subseteq}}
\newunicodechar{∩}{\ensuremath{\cap}}
\newunicodechar{∪}{\ensuremath{\cup}}
\newunicodechar{⊍}{\ensuremath{\uplus}}
\newunicodechar{⊎}{\ensuremath{\uplus}}

% \newunicodechar{⊤}{\ensuremath{\top}}
\newunicodechar{⊥}{\ensuremath{\bot}}
\newunicodechar{⊔}{\ensuremath{\sqcup}}
\newunicodechar{⊓}{\ensuremath{\sqcap}}
\newunicodechar{╲}{\ensuremath{\backslash}}

% \newunicodechar{╱}{\ensuremath{/}}

\newunicodechar{∘}{\ensuremath{\circ}}
\newunicodechar{↦}{\ensuremath{\mapsto}}
\newunicodechar{↪}{\ensuremath{\hookrightarrow}}

\newunicodechar{≠}{\ensuremath{\neq}}
\newunicodechar{≐}{\ensuremath{\doteq}}
\newunicodechar{≟}{\ensuremath{\stackrel{?}{=}}}
\newunicodechar{≅}{\ensuremath{\cong}}
\newunicodechar{≇}{\ensuremath{\ncong}}
\newunicodechar{≃}{\ensuremath{\simeq}}
\newunicodechar{≄}{\ensuremath{\not\simeq}}
\newunicodechar{≈}{\ensuremath{\approx}}
\newunicodechar{≉}{\ensuremath{\not\approx}}
\newunicodechar{∼}{\ensuremath{\sim}}
\newunicodechar{≁}{\ensuremath{\not\sim}}
\newunicodechar{≔}{\ensuremath{:\!=}}

\newunicodechar{≤}{\ensuremath{\leq}}
\newunicodechar{≰}{\ensuremath{\nleq}}
\newunicodechar{≥}{\ensuremath{\geq}}
\newunicodechar{≱}{\ensuremath{\ngeq}}
\newunicodechar{≮}{\ensuremath{\nless}}
\newunicodechar{≯}{\ensuremath{\ngtr}}
\newunicodechar{≦}{\ensuremath{\leqq}}
\newunicodechar{≨}{\ensuremath{\lneqq}}
\newunicodechar{≧}{\ensuremath{\geqq}}
\newunicodechar{≩}{\ensuremath{\gneqq}}
\newunicodechar{≲}{\ensuremath{\lesssim}}
\newunicodechar{≳}{\ensuremath{\gtrsim}}
\newunicodechar{⊏}{\ensuremath{\sqsubset}}
\newunicodechar{⊑}{\ensuremath{\sqsubseteq}}
\newunicodechar{⊐}{\ensuremath{\sqsupset}}
\newunicodechar{⊒}{\ensuremath{\sqsupseteq}}

\newunicodechar{∣}{\ensuremath{\mid}}

\newunicodechar{→}{\ensuremath{\rightarrow}}
\newunicodechar{⇨}{\ensuremath{\rightarrow}}
\newunicodechar{➩}{\ensuremath{\rightarrow}}
\newunicodechar{⟿}{\ensuremath{\rightsquigarrow}}
\newunicodechar{←}{\ensuremath{\leftarrow}}
\newunicodechar{↔}{\ensuremath{\leftrightarrow}}
\newunicodechar{↑}{\ensuremath{\uparrow}}
\newunicodechar{↓}{\ensuremath{\downarrow}}
\newunicodechar{⇊}{\ensuremath{\downarrow\downarrow}}
\newunicodechar{⟶}{\ensuremath{\longrightarrow}}
\newunicodechar{⟵}{\ensuremath{\longleftarrow}}

\newunicodechar{⊕}{\ensuremath{\oplus}}
\newunicodechar{⨁}{\ensuremath{\bigoplus}}
\newunicodechar{⊖}{\ensuremath{\ominus}}
\newunicodechar{⊗}{\ensuremath{\otimes}}
\newunicodechar{⨂}{\ensuremath{\bigotimes}}
\newunicodechar{⊘}{\ensuremath{\oslash}}
\newunicodechar{⊙}{\ensuremath{\odot}}
\newunicodechar{⨀}{\ensuremath{\bigodot}}
\newunicodechar{⊚}{\ensuremath{\circledcirc}}
\newunicodechar{⊛}{\ensuremath{\circledast}}
\newunicodechar{⊝}{\ensuremath{\circleddash}}

% \DeclareMathOperator{\VCCompose}{\longrightarrow\hspace{-3.5ex}\oplus\;}
% \newunicodechar{⟴}{\ensuremath{\!\!\VCCompose}}

% \newunicodechar{‼}{\ensuremath{!\!!}}
% \newunicodechar{∶}{\ensuremath{:}}

\newunicodechar{∙}{\ensuremath{\cdot}}
\newunicodechar{∞}{\ensuremath{\infty}}


\newunicodechar{✔}{\ensuremath{\checkmark}}
\newunicodechar{✓}{\ensuremath{\checkmark}}


\newunicodechar{□}{\ensuremath{QED}}
% +latex_header: 
\newunicodechar{∎}{\ensuremath{QED}}
\newunicodechar{○}{\ensuremath{\circ}}

\newunicodechar{♯}{\ensuremath{SHARP}}
% \newunicodechar{́}{\ensuremath{'}}
%% end-bebu



